Double trouble: Predicting new variant counts across two heterogeneous populations

Collecting genomics data across multiple heterogeneous populations (e.g., across different cancer types) has the potential to improve our understanding of disease. Despite sequencing advances, though, resources often remain a constraint when gathering data. So it would be useful for experimental design if experimenters with access to a pilot study could predict the number of new variants they might expect to find in a follow-up study: both the number of new variants shared between the populations and the total across the populations. While many authors have developed prediction methods for the single-population case, we show that these predictions can fare poorly across multiple populations that are heterogeneous. We prove that, surprisingly, a natural extension of a state-of-the-art single-population predictor to multiple populations fails for fundamental reasons. We provide the first predictor for the number of new shared variants and new total variants that can handle heterogeneity in multiple populations. We show that our proposed method works well empirically using real cancer and population genetics data.

==> tex/conjugacy.tex <==
% !TEX root = ../double_trouble_supp.tex

\subsection{Formal account on exponential family conjugacy}

%\begin{myDefinition}[Complete random measure and BNP prior]
    
%\end{myDefinition}
%\lom{Let's open the section saying what we prove in this section; I assume we want to say something along the lines of ``in this section we show that our proposed model enjoys some notion of conjugacy''}

In this section, building on the general the theory of completely random measures (or CRMs) and the results  developed by \citet{Broderick2018}, we prove that our proposed prior is conjugate with respect to two population Bernoulli process likelihood model.\footnote{\textcolor{red}{lom: but why does it matter?}} 
For a thorough account of CRMs, see \citet{kingman1967completely} and \citet[Chapter 8]{kingman1992poisson}.
We begin by restating the definition of exponential family and conjugacy of completely random measures [CRMs] provided in \citet{Broderick2018}. 

We first recall the definition of an exponential family likelihood 

We say the observation $x_\popidx|\variantfreqperpop{\popidx, \variantidx}$ are exponential family if

\begin{equation}
    h(x_\popidx|\variantfreqperpop{\popidx, \variantidx})dx_\popidx=\kappa_{\popidx}(x_\popidx)\exp\{ \left\langle\eta_{\popidx}(\variantfreqperpop{\popidx, \variantidx}), \phi_{\popidx}(x_\popidx)\right\rangle - A_{\popidx}(\variantfreqperpop{\popidx, \variantidx}) \}\mu_{\popidx}(dx_\popidx)
\end{equation}

We can check that independent two population Bernoulli are indeed exponential family. When the likelihood for two population $\popidx$ factorize, we observe that the joint likelihood condition on $\vecvariantfreq{\variantidx}=(\theta_{1,\variantidx},\dots)$ is still exponential family since sum of inner product is the inner product of concatenation. 

\begin{align}
    h(\bx|\vecvariantfreq{\variantidx})d\bx=\prod_{\popidx} h(x_\popidx|\variantfreqperpop{\popidx, \variantidx})dx_\popidx=\prod_{\popidx}\kappa_{\popidx}(x_\popidx) \exp\{ \sum_{\popidx} \left\langle\eta_{\popidx}(\variantfreqperpop{\popidx, \variantidx}), \phi_{\popidx}(x_\popidx)\right\rangle - \sum_{\popidx}A_{\popidx}(\variantfreqperpop{\popidx, \variantidx}) \}\prod_{\popidx}\mu_{\popidx}(dx_\popidx)
    \label{eq:exponential_likelihood_multiple_pop}
\end{align}

\citet{Broderick2018} extend it into complete random measures, we restate their definition below. 

\begin{myDefinition}[Exponential family CRM]
    A multivariate CRM is an exponential family with (fixed) functions $\kappa, \eta, \phi, A$ and members of this family are parameterized by $\zeta_k$ if:%\footnote{lom: is the CRM an exponential family or a member of the exp family?}
    \begin{itemize}
    	\item The fixed component is characterized by a collection of location, rate atoms $(\psi_{fix,k}, \vecvariantfreq{\text{fix},k})$, $k=1,2,\ldots$, where the locations $\psi_{fix,k}$ are all distinct and the the $k$-th random rate $\vecvariantfreq{\text{fix},k}$ has density
    \begin{equation*}
        f_{\text{fix},k}(\vecvariantfreq{})=\kappa(\vecvariantfreq{})\exp\{\left\langle \eta(\zeta_k),\phi(\vecvariantfreq{})\right\rangle -A(\zeta_k) \},
    \end{equation*}
    for a base measure $\kappa$, natural parameter function $\eta$ and sufficient statistics $\phi$. 
    \item For some $\mass>0$, the ordinary component is characterized by a rate measure $\levync(\de\vecvariantfreq{})$
    \begin{align*}
        \levync(\de\vecvariantfreq{})=\mass \exp\{\left\langle \eta(\zeta),\phi(\vecvariantfreq{})\right\rangle\}.
    \end{align*}
    \end{itemize}
    In particular we require $\eta$ and $\phi$ to be shared across the two components.
\end{myDefinition}

We notice that our proposed prior, introduced in \Cref{eq:proposed_prior}, can be viewed as a CRM with no deterministic, or fixed location component, i.e.\ only with an ordinary component.

\begin{myDefinition}[Exponential conjugacy of BNP prior] \label{def:conjugacy}
    We say that a CRM is an exponential conjugate BNP prior, if the posterior has fix location component and ordinary component in the same exponential family parameterization as the prior.\footnote{\lom{what is the role of the likelihood in this definition? I am a little confused here}}
\end{myDefinition}



\subsection{Our proposal is a  conjugate prior}

We now show that our proposed prior introduced in \Cref{eq:proposed_prior} when paired with the two-population Bernoulli process model yields a posterior that is conjugate in the sense of \Cref{def:conjugacy}.

\begin{myProposition}[Conjugacy]
    The proposed prior is a conjugate family to two population Bernoulli process such that 
    \begin{align*}
        h(x_{\popidx,\variantidx,\unitidx}|\variantfreqperpop{\popidx, \variantidx})dx_\popidx&=\prod_{\popidx} \variantfreqperpop{\popidx, \variantidx}^{x_{\popidx,\variantidx}}(1-\variantfreqperpop{\popidx, \variantidx})^{1-x_{\popidx,\variantidx}}\\
    \end{align*}
    And our prior has $\kappa = \frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}$, $\eta(\zeta) = \zeta - 1$, $\phi(\theta) = (\log(\variantfreqperpop{1}),\log(\variantfreqperpop{2}),\log(1-\variantfreqperpop{1}),\log(1-\variantfreqperpop{2}))$ parameterized by $\zeta = (\corr{1},\corr{2}, \conc{1}, \conc{2})$ and $A(\zeta)=\log(B(\corr{1}, \conc{1})B(\corr{2}, \conc{2})/\mass)$\footnote{\lom{i am again confused - should we not mention the likelihood model in the statement?}}
    \label{prop:conjugate}
\end{myProposition}

\begin{proof}
	\lom{deferring going over this until we chat  @yunyi, think it will be more efficient to walk over it together.}
	
    We write out the likelihood function of one atom and $N_{\popidx}$ samples in $\popidx$ population 
    \begin{align*}
        h(\bx|\vecvariantfreq{})&=\exp\left[\sum_{\popidx=1}^2(\sum_{\unitidx=1}^{N_{\popidx}}x_{\popidx,\unitidx}\log(\theta_{\popidx})+\sum_{\unitidx=1}^{N_{\popidx}}(1-x_{\popidx,\unitidx})\log(1-\theta_{\popidx}))\right]
    \end{align*}

    Though we assume no fixed location atoms in the prior, we could, define the family to have a set of fixed location atoms indexed by $k$, $\psi_{k,fixed}$ whose rate has distribution 
    \begin{align*}
        f_{prior, fixed, k}(\vecvariantfreq{})&\propto\frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}\exp\{\sum_{\popidx=1}^2 \xi_{\popidx,k,1}\log(\theta_{\popidx})+\xi_{\popidx,k,0}\log(1-\theta_{\popidx})\}
    \end{align*}
    There are such $\xi_{\popidx,k,1}$'s that make this normalizable e.g. when $\xi_{\popidx,k,0}>-1$ and $\xi_{\popidx,k,1}>\corr{\popidx}$ (which can be rewrite to $\variantfreqperpop{1}^{1+\xi_{1,k,1}-\corr{1}}\variantfreqperpop{2}^{1+\xi_{2,k,1}-\corr{2}}\levync(\de\vecvariantfreq{})$, which is normalizable by assumption of $\levync(\de\vecvariantfreq{})$).

    Then we have the posterior of the weight of the fixed atoms
    \begin{align*}
        f_{posterior, fixed, k}(\vecvariantfreq{})&\propto\frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}\exp\{\sum_{\popidx=1}^2 (\xi_{\popidx,k,1}+\sum_{\unitidx=1}^{N_{\popidx}}x_{\popidx,\unitidx,k})\log(\theta_{\popidx})\\
        &~~~~+(\xi_{\popidx,k,0}+\sum_{\unitidx=1}^{N_{\popidx}}(1-x_{\popidx,\unitidx,k}))\log(1-\theta_{\popidx})\}
    \end{align*}
    within the same family and new parameters $\xi_{\popidx,k,1}+\sum_{\unitidx=1}^{N_{\popidx}}x_{\popidx,\unitidx,k}, \xi_{\popidx,k,0}+\sum_{\unitidx=1}^{N_{\popidx}}(1-x_{\popidx,\unitidx,k})$. 

    We write the ordinary component of our prior in exponential form
    \begin{align*}
        \nu(\vecvariantfreq{})&=
        \frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}\exp\{\sum_{\popidx=1}^2 (\corr{\popidx}-1)\log(\theta_{\popidx})+(\conc{\popidx}-1)\log(1-\theta_{\popidx}) -\log(B(\corr{1}, \conc{1})B(\corr{2}, \conc{2})/\mass) \}
        \de\vecvariantfreq{}
    \end{align*}

    Thus for new atoms $\delta_{\psi_{\text{new}, k}}$ the posterior has a fix location components with weight distribution 
    \begin{align*}
        f_{post, \text{new}, k}(\vecvariantfreq{})&\propto \levync(\de\vecvariantfreq{})\cdot h(\bx_{\text{new}, k}|\vecvariantfreq{})\\
        &\propto \frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}\exp\{\sum_{\popidx=1}^2 (\corr{\popidx}+\sum_{\unitidx=1}^{N_{\popidx}}x_{\popidx,\unitidx,\text{new}, k}-1)\log(\theta_j)\\
        &~~~~+(\conc{\popidx}+\sum_{\unitidx=1}^{N_{\popidx}}(1-x_{\popidx,\unitidx,\text{new}, k})-1)\log(1-\theta_j) \}
    \end{align*}
    and the ordinary component
    \begin{align*}
        \nu(\vecvariantfreq{})\cdot h(0|\vecvariantfreq{})&=\frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}\exp\{\sum_{\popidx=1}^2 (\corr{\popidx}-1)\log(\theta_j)\\
        &~~~~+(\conc{\popidx}+1-1)\log(1-\theta_j) -\log(B(\corr{1}, \conc{1})B(\corr{2}, \conc{2})/\mass) \}
        \de\vecvariantfreq{}
    \end{align*}
    Within the same family of our prior, since we have the sufficient statistics are shared across the ordinary and fixed components in the posterior and a non-factorized base measure $\frac{(\variantfreqperpop{1}+\variantfreqperpop{2}^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\variantfreqperpop{1}+\variantfreqperpop{2})^{\corr{1}+\corr{2}}}$
\end{proof}


\subsection{On automatic conjugacy by \citet{Broderick2018}} 

%\lom{Is the idea of this section that we can't rely on automatic conjugacy? Unless we state here explicitly this, I think this section seems confusing, in the sense that ``automatic conjugacy'' is still a relatively niche concept most people wont be familiar with. I would propose also to move this at the end of the section, if it is not needed to show our main point (that is, our prior is conjugate)}

One might ask whether our proposed prior is a special case of automatic conjugate prior proposed by \citet{Broderick2018}. It is actually not, more over, we hereby show in this multiple population case the constructed prior following procedure of~\citet{Broderick2018} has to be product measure. 

We can directly apply Theorem 4.2 from \citet{Broderick2018} to conclude their automatic conjugate prior must be a factorized, as~\Cref{coro:conjugate_is_product}.

\begin{myCorollary}
    \label{coro:conjugate_is_product}
    The automatic conjugate prior by \citet{Broderick2018} for factorized exponential family likelihood is factorized. 
\end{myCorollary}

\begin{proof}
    Directly apply Theorem 4.2 from \citet{Broderick2018} to the likelihood~\eqref{eq:exponential_likelihood_multiple_pop}. The rate measure of conjugate prior take the form 
    \begin{align*}
        \levync(\de\vecvariantfreq{})=\mass \exp\{ \sum_{\popidx}\left\langle\xi_{\popidx}, \eta_{\popidx}(\theta_{\popidx})\right\rangle-\lambda \sum_{\popidx}A_{\popidx}(\theta_{\popidx}) \}=\mass \prod_{\popidx} \exp\{ \left\langle\xi_{\popidx},  \eta_{\popidx}(\theta_{\popidx})\right\rangle-\lambda A_{\popidx}(\theta_{\popidx}) \}
    \end{align*}
    which factorized.
\end{proof}


==> tex/extensions.tex <==
% !TEX root = ../double_trouble_main.tex
\paragraph{Conjugate prior in exponential family}

\citet{Broderick2018} described a large class of Bayesian nonparametric priors for exponential family likelihoods. That is, suppose data condition on random parameter $\theta$ has distribution $H(dx|\theta)$ take the form
\begin{align*}
    H(dx|\theta)=\kappa(x)\exp\left[\left\langle \eta(\theta), \phi(x)\right\rangle -A(\theta) \right]
\end{align*}

A natural BNP prior can be expressed as a CRM with ordinary components of form
\begin{align}
    \nu(d\theta)=\gamma \exp\left[\left\langle\xi, \eta(\theta)\right\rangle-\lambda A(\theta)\right]
\end{align}
where $\gamma, \xi, \lambda$ are chosen to satisfy the finite expectation and infinite mass assumption. 

While conjugacy is a nice property, unfortunately when the likelihood factorize in two populations, the conjugate prior will be a product measure. 

\begin{myProposition}[No conjugate prior for factorized exponential family]
    Suppose the exponential likelihood factorize, i.e. the likelihood 
    \begin{align*}
        H(d\bx|\btheta)=\prod_i \kappa_i(x_i)\exp\left[\sum_{i} \left\langle \eta_i(\theta_i), \phi_i(x)\right\rangle -A_i(\theta_i) \right]
    \end{align*}
    Then there is no proper conjugate CRM prior
\end{myProposition}
\begin{proof}
    We observe that the likelihood still in exponential family by writing sum of inner product as a inner product of concatenations. Follow Theorem 4.2 of \citet{Broderick2018}, we have the unique conjugate prior family being
    \begin{align*}
        \nu(d\btheta)=\gamma \exp\left[\sum_i \left\langle\xi_i, \eta_i(\theta_i)\right\rangle-\lambda_i A_i(\theta_i)\right]
    \end{align*}
    which is itself a product measure thus cannot be proper. 
\end{proof}


\paragraph{Some extensions of the near conjugate priors}
However, our method when $\alpha_1=\alpha_2$, i.e. having a leading term of $(\theta_1+\theta_2)^{a}$ in front of a proper conjugate distribution for some carefully chosen $a$ might provide a general strategy of constructing ``near conjugate'' priors when $\eta_i=\eta$ and $A_i=A$ are monotone. I.e., we consider the family of prior that have
\begin{align*}
    \nu(d\btheta)=\gamma \exp\left[\sum_i \left\langle\xi_i, \eta(\theta_i)\right\rangle-\lambda_i A(\theta_i)\right]\exp\left[\tau \eta(\sum_i\theta_i)\right]
\end{align*}
This formulation is convenient since we always have the bound that $\theta_i\le \sum_{i=1}^J \theta_i\le J\max\{\theta_i\}$ thus searching for $\tau$ can be reduce to the similar process of searching for conjugate priors. We have the conjugate part enable a simple MC evaluation of integrals. 

We give some examples

\begin{myExample}[Gamma]
For a Poisson likelihood process, whose likelihood $h(x|\theta)=\theta^xe^{-\theta}/x!$. The one dimensional conjugate prior has rate measure $\gamma\theta^\xi e^{-\lambda\theta}$ with $\xi\in(-2,-1]$ and $\lambda>0$. For a two dimensional case, we consider a family $\gamma(\theta_1+\theta_2)^{\tau}\theta_1^{\xi_1-1}\theta_2^{\xi_2-1} e^{-\lambda_1\theta_1-\lambda_2\theta_2}$. We need $\lambda_1,\lambda_2>0$ to control when $\theta\in[\epsilon,\infty)$ for some small $\epsilon$. For $\theta\in (0,\epsilon)$ when can show that if $\xi_1,\xi_2>0$, $-\tau\in (\xi_1+\xi_2,\xi_1+\xi_2+1)$, the prior is proper. 
\end{myExample}

\begin{myExample}[Beta prime]
    The beta prime processes were introduce by \citet{Broderick2018}, whose likelihood is given by the odds $h(x|\theta)=\theta^x(1-\theta)^{-1}$. Suppose the bivariate version factorize, we have $h(\bx|\btheta)=\theta_1^{x_1}(1-\theta_1)^{-1}\theta_2^{x_2}(1-\theta_2)^{-1}$. The one dimensional prior has rate measure $\gamma\theta^\xi(1+\theta)^{-\lambda}$. We can consider a rate measure $\gamma(\theta_1+\theta_2)^\tau\theta_1^{\xi_1}(1+\theta_1)^{-\lambda_1}\theta_2^{\xi_2}(1+\theta_2)^{-\lambda_2}$. It is simple to check when $\lambda_1,\lambda_2>0$, $\xi_1,\xi_2>-1$ and $-\tau\in (\xi_1+\xi_2,\xi_1+\xi_2+1)$ the prior is proper. 
\end{myExample}



==> tex/fitting.tex <==
% !TEX root = ../double_trouble_supp.tex

In this section we discuss the empirics we adopt to fit the hyperparameters of the competing baselines d3BP and i3BP. 
%These procedures are similar. 

\subsection{Fitting the hyperparameters of the d3BP}

For the d3BP, we adopt an approach closely related to the one described in the main text in \Cref{sec:hyperparameter_empirics}. 
In particular, similar to~\Cref{eq:likelihood_prior}, we define the following objective function:
\begin{equation}
    \label{eq:appx_likelihood_prior}
    \mathcal{L}(\{\mass, \conc{}, \discount{}\})=
    	\sum_{\substack{\vecoccurrence: \occurrence{1},\occurrence{2} \in 0:v \\ \occurrence{1} + \occurrence{2} \ge 1}}
		\log \left[ \pois \left(
				\obsnews{\vecsamplesize_\train}{\vecsamplesize - \vecsamplesize_\train, \vecoccurrence}
				\mid \lambda^{(\vecsamplesize - \vecsamplesize_\train,\bm{k})}_{\mathrm{d3BP},\vecsamplesize_\train}(\{\mass, \conc{}, \discount{}\})
			\right) \right],
\end{equation}
where $\lambda^{(\vecsamplesize - \vecsamplesize_\train,\bm{k})}_{\mathrm{d3BP},\vecsamplesize_\train}(\{\mass, \conc{}, \discount{}\})$ was defined in \Cref{prop:kr_ton_diag}, and we here emphasize its dependence on the hyperparameters $\mass, \conc{}, \discount{}$.

%Similarly, from the training set of size $N=(N_1,N_2)$, we condition on a minitrain of size $N_0=(N_{1,0},N_{2,0})$, in our experiments we chose $N_{1,0}=N_1/2, N_{2,0}=N_2/2$. We can calculate the observed number of \textit{new} variants (after minitrain set) exist $\ell=(\ell_1,\ell_2)$ times $u^{(N-N_0,\ell)}_{N_0}$. We can treat these as the prediction when there is a pilot data of size $(N_{1,0},N_{2,0})$. By Following \citet{Masoero2022}, we can show that the posterior distribution of $\ell$-tons condition on the minitrain set is Poisson with mean 
%\begin{align*}
%    \newsparam{\vecsamplesize_\train}{\vecsamplesize - \vecsamplesize_\train, \vecoccurrence}(\allhyper)=\alpha\binom{\samplesize{1}-\samplesize{1,\train}}{\occurrence{1}}\binom{\samplesize{2}-\samplesize{2,\train}}{\occurrence{2}}\frac{(1-\sigma)_{(\occurrence{1}+\occurrence{2})\uparrow}(c+\sigma)_{(\samplesize{1}+\samplesize{2}-\occurrence{1}-\occurrence{2})\uparrow}}{(c+1)_{(\samplesize{1}+\samplesize{2}-1)\uparrow}}
%\end{align*} 

In our experiments, we initialize the algorithm\footnote{\lom{which algorithm though? let's spell it out. and why these values?}} with $(\alpha, \sigma, c)=(10^3, 0.5, 1)$.

%The objective function is given by the log likelihood
%\begin{equation}
%    \label{eq:likelihood_prior}
%    \mathcal{L}(\gamma, \alpha, \sigma_1,\sigma_2, c_1,c_2)=\sum_{\ell_1=1}^v\sum_{\ell_2=0}^v\log\left[\text{pois}\left(u^{(N-N_0,\ell)}_{N_0}\vert \lambda^{(N-N_0,\ell)}_{N_0}\right)\right]+\sum_{\ell_2=1}^v\log\left[\text{pois}\left(u^{(N-N_0,\ell)}_{N_0}\vert \lambda^{(N,(0,\ell_2))}_{0}\right)\right]
%\end{equation}
%Then we set the hyperparameter to be 
%\begin{align*}
%    ( \hat\alpha, \hat\sigma, \hat c)=\argmax \mathcal{L}(\alpha, \sigma,c_2)
%\end{align*}

This procedure also provide a method to fit 3BP by randomly dividing the population into two and fit a d3BP. An alternative way to view this procedure to fit a 3BP hyperparameter is that we take two snapshot in time and predict number of k-tons, while the training procedure in \citet{Masoero2022} is predicting singletons in all snapshot in time. \footnote{\lom{i can't understand this paragraph}}


\subsection{Fitting i3BP with two least square}


For the i3BP, in which the two populations are treated as independent, we use the method described in \citet[Equation 6]{Masoero2022}. I.e., we randomly split the training set in two parts, a ``minitrain'' part in which we retain $2/3$ of the data, and find the hyperparameter values that best predict the rate of growth of the number of new variants on the remaining 1/3 of the training set. In this case, the objective function is the $\ell_2$ loss between the predicted number of new variants and the actual number of new values. 
Alternatively we fit a d3BP on two randomly split subpopulation on each population to form an i3BP. \footnote{\lom{do we adopt this alternative though?}}

==> tex/method.tex <==
% !TEX root = ../double_trouble_main.tex

We start by reviewing the Bayesian nonparametric (BNP) framework used for the optimal experimental design problem sketched in \Cref{sec:intro} when only one population is present.
We assume to have a collection of $M$ genomes from a single population. For each genome, we can determine if the nucleotide at each locus agrees (i.e., no variant) or disagrees (i.e., variant) with a underlying fixed, known reference genome. 

Suppose that a total of $L$ distinct loci disagree with the reference genome across the $M$ samples.
%\footnote{\lom{``Suppose that a total of $L$ distinct loci disagree with the reference genome across the $M$ samples.''}\yunyi{I agree. A concern: we need to turn to the ``variant'' for loci sometime soon, not sure when it will be good or it is ok as is. }} 
We then let $\Omega$ be some arbitrary sample space of variant labels, with $\psi_{\ell}$ the label for the $\ell$-th variant observed. For the $n$-th individual, let $x_{n,\ell}=1$ equal 1 if the variant with label $\psi_\ell$ is observed for the $n$-th organism in population, and $x_{n,\ell}=0$ otherwise. Denote $\delta_A(x)$ as the Dirac measure at $A$, i.e.\ $\delta_A(x) = 1(x\in A)$. The $n$-th genome can then be represented as a measure $X_{n}=\sum_{\ell=1}^Lx_{n,\ell}\delta_{\psi_\ell}.$
%\footnote{\lom{worth pointing out $\delta_A(x)$ is the Dirac mass at $A$, i.e.\ $\delta_A(x) = 1(x\in A)$.}\yunyi{yeah}} 
We adopt a Bernoulli product model, in which each $X_{n,\ell}|\bTheta_0\sim\Bernoulli(\theta_{\ell})$, independent across loci $\ell=1,\ldots,L$ and i.i.d.\ across samples $n=1,\ldots,M$. Further, we endow the rates with a nonparametric prior distribution.

That is, we imagine that there exist countably many of variants and collect the rate-variant pair using a (scalar-valued) random measure $\Theta_0=\sum_{\ell=1}^\infty \theta_\ell\delta_{\psi_\ell}$.  The rates $\{\theta_\ell\}\subset[0,1]$ can be modeled as draws from the three-parameter-Beta process (3BP, \citet{Masoero2022}) where they model the $\theta_\ell$ being generated by a Poisson process on unit interval that has infinite mass and finite expectations.




Let us assume now to have collected genomic data from $I = 2$ population of cancer cells, each population indexed by $i$. Let $L$ denote the total distinct variants observed across  the $I$ populations. We represent the $n$-th genome in the $i$-th population via the measure $X_{i,n}=\sum_{\ell=1}^Lx_{i,n,\ell}\delta_{\psi_\ell}$. Notice that the labels $\psi_\ell$ are ``matched'', i.e.\ shared across the multiple populations. The rate of a given variant could be
%\footnote{\lom{I don't think we want to say it \emph{should} be done this way, rather that's what we propose} \yunyi{true..., I changed it to could}} 
modeled as a \textit{vector} $\btheta_\ell$ whose entries are the frequency of the variant in each population. That is, we collect the rate-variant pair in a vector valued random measure $\bTheta_0=\sum_{\ell=1}^\infty \btheta_\ell\delta_{\psi_\ell}$ and model $x_{i,n,\ell}|\bTheta_0\sim \Bernoulli(\theta_{i,\ell})$ conditionally independent.
%\footnote{\lom{might want to condition on $\Theta_0$ and say what is independent of what}\yunyi{yes}}. 
In this way we model each variant to have multiple rate accounting for different populations. Our main idea is to model the rate-variant pair $\bTheta_0=\sum_{\ell=1}^\infty \btheta_\ell\delta_{\psi_\ell}$ analogous to the 3BP, by defining a Poisson process on the unit square
%\footnote{\lom{not clear whether $\Omega = [0,1]$ here. I wonder if we could say we model the frequencies as a PP on the unit square instead?}\yunyi{I think so, given we already say $I=2$}} 
with each variant being a point. In two dimension this is analogous to the \textit{frequency spectrum} \citep{Gutenkunst2009}. We would like the model to be a proper Bayesian nonparamatric (BNP) prior, that is, it should have infinite mass and finite expectations on each axis \citep{Broderick2018} thus be able to 1) have infinite amount of potential variants and 2) predict finite number of variants when any finite sample is taken from the two population. These two requirements also guarantee that the prior defines proper BNP priors by projecting to each axis thus able to handle ths situation that only one population was observed. 
%\footnote{\lom{I guess this is also to ensure some notion of consistency? two proposals: we lay out the desiderata for our model first -- i.e.\ (a) be a valid prior (infinite mass, finite expectations, see last year's workshop) and (b) have valid projections. other option, start by saying that the simplest thing is to take the product of the two measures, but this violates the projection property, which is a necessary consistency requirement?}\yunyi{actually (a) and (b) are kinda the same, because the expectations are defined on each axis so the double integral can be understood as first calculate the projection process and then make sure they are proper}} 

The most straightforward proposal to construct a measure on unit square with infinite mass was to define the Poisson process with rate measure being a product measure of e.g. two 3BP's. Unfortunately one can show any product measure having more than one non-$\delta$ measure cannot have finite expectation on all axes (see Appendix.\ref{sec:product_measure}). The consequence is that there exist some finite sampling schemes that the model will make unrealistic prediction of seeing infinite number of variants. Another simple yet useful model is the ``diagonal measure'' where we model $\theta_1=\theta_2$ as a 3BP. However this model essentially view the two populations as one thus no heterogeneity is accounted. We would like a model in between: that have proper normalization and allow heterogeneity. To allow heterogeneity, we would like a rate measure to have support on the entire unit square.
%\footnote{\lom{I like that you list these two options upfront. To me these are kind of opposite simple approaches, and we have good reasons why neither of these is really satisfactory: in the first case you can't enforce consistency, in the latter you can't model heterogeneity. Maybe we could rephrase emphasizing these things as a motivation for why we need to create a more complicated model that interpolates between these two simple options?}\yunyi{That is a good idea and I need little more time on it. Mark as TODO}}  
One can construct infinitely many such measures but not everyone of them are easy to work with. One important feature makes 3BP easy is that it is conjugate to Bernoulli likelihood \citep{Broderick2012,Broderick2018}, i.e. the prior and posterior take the same function form and updating can be done via algebraic calculations. While we cannot take product measure to keep the conjugacy perfectly, we hope to still mostly keep the updating algebraic and support the entire unit square.  
%\footnote{\lom{I think we might want to be precise here. Conjugacy is a binary attribute --- what do we mean by mostly keep the conjugacy?}\yunyi{yes}} 
We proposed a ``near conjugate'' priors in two dimension that are Poisson processes with rate measure $\nu(\btheta)=\frac{\gamma}{B(\sigma_1,c_1)B(\sigma_2,c_2)}(\theta_1+\theta_2)^{-\alpha-\sigma_1-\sigma_2}\theta_1^{\sigma_1-1}\theta_2^{\sigma_2-1}(1-\theta_1)^{c_1-1}(1-\theta_2)^{c_2-1}$ where $B()$ is the beta function. If $\gamma,\sigma_1,\sigma_2,c_1,c_2>0$ and $\alpha\in(0,1)$ this rate measure are infinite in mass and has finite expectation for both coordinates thus being a proper BNP prior. The rate measure takes a beta form up to a non-constant factor $(\theta_1+\theta_2)^{-\alpha-\sigma_1-\sigma_2}$, which make the posterior take a similar functional form. Roughly $\alpha$ controls the growth curve while $\sigma_1,\sigma_2$ control the form of correlations (Fig.\ref{}) and $c_1,c_2$ controls the ``common'' variants and $\gamma$ is a scaling factor on number of variants one would expect to see. 
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{Figs/rate_measures_near_cojugate.png}
    \caption{Log10 rate measure with different $\sigma_1,\sigma_2$ values. The hyperparameters $\sigma_1$ and $\sigma_2$ controls the form of correlations between axes. }
\end{figure}

%\footnote{\lom{I think if we introduced this as a model desideratum earlier, it'd be clearer why we care about it in this context}\yunyi{true, I tried}}. 
Although in the present work we focus on the two populations ($I=2$), extensions to any finite number $I$ of populations is straightforward by define the Poisson process on unit-cube with rate measure being  $(1^\top \btheta)^{-\alpha-\sum_i \sigma_i}\prod_{i=1}^I\frac{1}{B(\sigma_i,c_i)}\theta_i^{\sigma_i-1}(1-\theta_i)^{c_i-1}$
In the next part of this paper we will test the performance of this proposal with some existing alternatives. 

==> tex/power_law-old.tex <==


Contrast with unidimensional situations, there are multiple ways we have $t\to\infty$ (resp. $\samplesize{}\to\infty$), we mainly consider two ways: 1) projection: with $t=(0,t_2)$ with $t_2\to \infty$ (resp. $\samplesize{}=(0,\samplesize{2})$ with $\samplesize{2}\to\infty$) or $t=(t_1,0)$ and $t_1\to\infty$ (resp. $\samplesize{}=(\samplesize{1},0)$ with $\samplesize{1}\to\infty$) and 2) proportional sampling, i.e. $\samplesize{}=(\samplesize{1}, a\samplesize{1})$. Since the power law is asymptotic, situation 1 generalize to the situation that has finite sample in one population and the other diverge. 

\subsection{Power law bounds in projection scheme}
\label{sec:projection_scheme_proof}
Here we give the proof of~\Cref{prop:power_law_proj}.

\begin{proof}
    
For the projection scheme, we can focus on the population being sampled. The variants' frequency came from the ``projection'' of the two dimensional rate measure by integrating the other population out. We can then check the conditions in \citet{Broderick2012} in the projection rate measure, i.e. we want 
\begin{align*}
    \int_0^x\int_0^1\theta_i\nu(d\btheta)\sim \frac{\rate{i}}{1-\rate{i}}x^{1-\rate{i}}l(1/x)
\end{align*}
For some regularly varying function $l$ and $\rate{i}\in(0,1)$. We check this for the near conjugate prior. However we do not have the analytical solution of this integral, we target on bounding it with similar rates. Without lose of generality, we consider $\theta_1$, for a small $\delta>0$. 
\begin{align*}
    &\int_0^x\int_0^1 \theta_1\nu(d\btheta)\\
    =&\int_0^x\int_0^1 \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}\\
    \le&\int_{0}^x\int_0^1 \theta_1^{-\rate{1}-\corr{i}-\delta}\theta_1^{\corr{i}}\theta_2^{-\corr{2}+\delta}\theta_2^{\corr{2}-1} d\btheta\\
    =&\int_{0}^x\int_0^1 \theta_1^{-\rate{1}-\delta}\theta_2^{\delta-1}d\btheta\\
    =&\int_{0}^x\theta_1^{-(\rate{1}+\delta)}d\theta_1\\
    \sim& \frac{1}{1-(\rate{1}+\delta)} x^{1-(\rate{1}+\delta)}\\
    \to &  \frac{1}{1-\rate{1}} x^{1-(\rate{1})}\\
\end{align*}
We used the fact that $\theta_1+\theta_2\ge \theta_1,\theta_2$. By assumption of $\rate{}$ and $\sigma$'s, for small enough $\delta$, we have $\rate{}+\delta\in (0,1)$. Now we need a lower bound by the same rate. We use the fact that $\theta_1+\theta_2\le 2\max \{\theta_1,\theta_2\}$. We bound by integrating over only range $\theta_1\ge \theta_2$ if $\rate{2}\ge \rate{1}$, we have $\theta_1\ge \theta_2\ge \theta_2^{\rate{2}/\rate{1}}$

\begin{align*}
    &\int_0^x\int_0^1 \theta_1\nu(d\btheta)\\
    =&\int_0^x\int_0^1 \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}d\btheta\\
    \ge & \int_0^x\int_0^{\theta_1} \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}d\btheta\\
    \ge& 2^{-\rate{1} -\corr{i}-\corr{2}}\int_0^x\int_0^{\theta_1} \theta_1^{-\rate{1}-\corr{i}-\corr{2}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}d\btheta\\
    \sim &2^{-\rate{1}-\corr{i}-\corr{2}}  \int_0^x\int_0^{\theta_1} \theta_1^{-\rate{1}-\corr{i}-\corr{2}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}d\theta_2d\theta_1\\
    =&\frac{2^{-\rate{1}-\corr{i}-\corr{2}}}{\corr{2}}\int_0^x \theta_1^{-\rate{1}}d\theta_1\\
    =&\frac{2^{-\rate{1}-\corr{i}-\corr{2}}}{\corr{2}}\frac{1}{1-\rate{1}} x^{1-\rate{1}}
\end{align*}

For $\rate{2}\le \rate{1}$ ($\rate{2}/\rate{1}\le 1$) we integrating over the range $\theta_1\ge \theta_2^{\rate{2}/\rate{1}}\ge \theta_2$ we cannot get the lower bound to be the same

\begin{align*}
    &\int_0^x\int_0^1 \theta_1\nu(d\btheta)\\
    \ge&\int_0^x\int_0^{\theta_1^{\rate{1}/\rate{2}}} \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}d\btheta\\
    \sim & \int_0^x\int_0^{\theta_1^{\rate{1}/\rate{2}}} \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}d\btheta\\
    \ge & 2^{-\rate{1}-\corr{i}-\corr{2}} \int_0^x\theta_1^{-\rate{1}-\corr{2}}\int_0^{\theta_1^{\rate{1}/\rate{2}}} \theta_2^{\corr{2}-1}d\btheta\\
    %\ge & \int_0^x\theta_1^{-\rate{1}-\corr{2}}\int_0^{\theta_1^{\rate{1}/\rate{2}}} \theta_2^{\corr{2}\frac{\rate{2}}{\rate{1}}-1}d\btheta\\
    =&2^{-\rate{1}-\corr{i}-\corr{2}}\int_0^x\theta_1^{-\rate{1}+\corr{2}(\frac{\rate{1}}{\rate{2}}-1)}d\theta_1
\end{align*}
%The key modification in the second of the last line used the fact that $\theta_2\le 1$ and $\corr{2}>0$. For $\theta_2$, we take the same argument, with modification on ranges. 



For $\rate{2}\le \rate{1}$ ($\rate{2}/\rate{1}\le 1$), an alternative way to find a lower bound is to first apply $(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}\ge (\theta_1^{\rate{2}/\rate{1}}+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}$ integrating over the range $\theta_1\ge \theta_2$ we can lower bound the rate using $\rate{2}$

\begin{align*}
    &\int_0^x\int_0^1 \theta_1\nu(d\btheta)\\
    \ge&\int_0^x\int_0^{\theta_1} \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}(1-\theta_1)^{\conc{1}-1}(1-\theta_2)^{\conc{2}-1}d\btheta\\
    \sim & \int_0^x\int_0^{\theta_1} \frac{(\theta_1+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}d\btheta\\
    \ge &\int_0^x\int_0^{\theta_1} \frac{(\theta_1^{\rate{2}/\rate{1}}+\theta_2^{\rate{2}/\rate{1}})^{-\rate{1}}}{(\theta_1+\theta_2)^{\corr{i}+\corr{2}}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}d\btheta\\
    \ge &2^{-\rate{1}-\corr{i}-\corr{2}}\int_0^x\int_0^{\theta_1} \theta_1^{-\rate{2}-\corr{i}-\corr{2}}\theta_1^{\corr{i}}\theta_2^{\corr{2}-1}d\btheta\\
    \ge &2^{-\rate{1}-\corr{i}-\corr{2}} \int_0^x\theta_1^{-\rate{2}-\corr{2}}\int_0^{\theta_1} \theta_2^{\corr{2}-1}d\btheta\\
    %\ge & \int_0^x\theta_1^{-\rate{1}-\corr{2}}\int_0^{\theta_1^{\rate{1}/\rate{2}}} \theta_2^{\corr{2}\frac{\rate{2}}{\rate{1}}-1}d\btheta\\
    =&2^{-\rate{1}-\corr{i}-\corr{2}}\int_0^x\theta_1^{-\rate{2}}d\theta_1
\end{align*}


Since $\delta$ arbitrary, we have there exist a function $f(\rate{},\sigma,c)$ such that  $\mass 2^{-\rate{}-\corr{i}-\corr{2}}/\corr{2}\le f \le \mass$ which must be regularly varying. Thus by proposition 6.1 in \citet{Broderick2012}, we have when $\rate{2}\ge \rate{1}$
\begin{align*}
    &\Phi((t_1,0))\sim  \mass(1-\rate{1})t_2^{\rate{1}}l(1/t_1), t_1\to\infty\\
    \mass(1-\rate{2}+\corr{i}(\rate{2}/\rate{1}-1))t_2^{\rate{2}-\corr{i}(\rate{2}/\rate{1}-1)}l(1/t_2)\lesssim&\Phi((0,t_2))\lesssim \mass(1-\rate{2})t_2^{\rate{2}}l(1/t_2), t_2\to\infty\\
    %\Phi_{(k_1,0)}((t_1,0))&\sim \frac{\rate{1}\mass(k_1-\rate{1})}{k_1!}t_1^{\rate{1}}l(t_1), t_1\to\infty, k_i>0\\
    %\Phi_{(0,k_2)}((0,t_2))&\sim \frac{\rate{2}\mass(k_2-\rate{2})}{k_2!}t_2^{\rate{2}}l(t_2), t_2\to\infty, k_2>0
\end{align*} 

we have when $\rate{2}\le \rate{1}$
\begin{align*}
    \mass(1-\rate{1}+\corr{2}(\rate{1}/\rate{2}-1))t_1^{\rate{1}-\corr{2}(\rate{1}/\rate{2}-1)}l(1/t_1)\lesssim&\Phi((0,t_1))\lesssim \mass(1-\rate{1})t_1^{\rate{1}}l(1/t_1), t_1\to\infty\\
    &\Phi((t_2,0))\sim  \mass(1-\rate{2})t_2^{\rate{2}}l(1/t_2), t_2\to\infty\\
    %\Phi_{(k_1,0)}((t_1,0))&\sim \frac{\rate{1}\mass(k_1-\rate{1})}{k_1!}t_1^{\rate{1}}l(t_1), t_1\to\infty, k_i>0\\
    %\Phi_{(0,k_2)}((0,t_2))&\sim \frac{\rate{2}\mass(k_2-\rate{2})}{k_2!}t_2^{\rate{2}}l(t_2), t_2\to\infty, k_2>0
\end{align*} 


Thus we have when $\rate{1}\le \rate{2}$
\begin{align*}
    &\news{\bm{0}}{(\samplesize{1},0)}\sim \conc{1} \samplesize{1}^{\rate{1}}\\
    \conc{2}'\samplesize{2}^{\rate{2}-\corr{i}(\rate{2}/\rate{1}-1)}\lesssim &\news{\bm{0}}{(0,\samplesize{2})} \lesssim \conc{2}\samplesize{2}^{\rate{2}}
\end{align*}
and when $\rate{1}\ge \rate{2}$

\begin{align*}
    \conc{1}'\samplesize{1}^{\rate{1}-\corr{2}(\rate{1}/\rate{2}-1)}\lesssim &\news{\bm{0}}{(0,\samplesize{1})} \lesssim \conc{1}\samplesize{1}^{\rate{1}}\\
    &\news{\bm{0}}{(\samplesize{2},0)}\sim \conc{2} \samplesize{2}^{\rate{2}}\\
\end{align*}

\end{proof}

\subsection{Power law bounds in proportional scheme}
\label{sec:proportion_scheme_proof}
Here we give the proof of~\Cref{coro:proportional}.

\begin{proof}
For a proportional sample $(\samplesize{1},\samplesize{2})=(\samplesize{},a\samplesize{})$ with $a>0$ and $\samplesize{}\to\infty$. We can bound the number of new variants $\news{\bm{0}}\samplesize{}$ by
\begin{align*}
    \max\{\news{\bm{0}}{(\samplesize{},0)},\news{\bm{0}}{0,a\samplesize{}}\}\le \news{\bm{0}}{(\samplesize{},a\samplesize{})}\le \news{\bm{0}}{(\samplesize{},0)}+\news{\bm{0}}{(0,a\samplesize{})}\le 2\max\{\news{\bm{0}}{(\samplesize{},0)},\news{\bm{0}}{0,a\samplesize{}}\}
\end{align*}
Use the result in projection scheme, we have when $\samplesize{}$ large the lower bound is further lower bounded by
\begin{align*}
    \max\{\news{\bm{0}}{(\samplesize{},0)},\news{\bm{0}}{0,a\samplesize{}}\} &\ge \max\{ \conc{1}\samplesize{}^{\rate{1}}, \conc{2}a^{\rate{2}}\samplesize{}^{\rate{2}} \}\ge \max\{\min\{\conc{1},\conc{2}a^{\rate{2}}\}\samplesize{}^{\rate{1}}, \min\{\conc{1},\conc{2}a^{\rate{2}}\}\samplesize{}^{\rate{2}}\}\\
    &\ge  \min\{\conc{1},\conc{2}a^{\rate{2}}\}\max\{\samplesize{}^{\rate{1}}, \samplesize{}^{\rate{2}}\}\\
    &=\min\{\conc{1},\conc{2}a^{\rate{2}}\}\samplesize{}^{\max\{\rate{1},\rate{2}\}}\\
    &=\frac{\min\{\conc{1},\conc{2}a^{\rate{2}}\}}{(1+a)^{\max\{\rate{1},\rate{2}\}}}(\samplesize{1}+\samplesize{2})^{\max\{\rate{1},\rate{2}\}}
\end{align*}
Similarly we have 
\begin{align*}
    2\max\{\news{\bm{0}}{(\samplesize{},0)},\news{\bm{0}}{0,a\samplesize{}}\}\le \frac{2\max\{\conc{1},\conc{2}a^{\rate{2}}\}}{(1+a)^{\max\{\rate{1},\rate{2}\}}}(\samplesize{1}+\samplesize{2})^{\max\{\rate{1},\rate{2}\}}
\end{align*}
That is, the total number of variants shows a power-law over total number of samples. 
\end{proof}

\subsection{Power law when $\rate{1}=\rate{2}=\rate{}$}
\label{sec:two_rate_the_same}
We give proof of~\Cref{coro:rate_align} when $\rate{1}=\rate{2}=\rate{}$.



\begin{proof}
    We use the same bound from proportional scheme with $\rate{1}=\rate{2}=\rate{}$
    \begin{align*}
        \max\{ \news{\bm{0}}{\samplesize{1},0},\news{\bm{0}}{0,\samplesize{2}}\} \le \news{\bm{0}}{\samplesize{1},\samplesize{2}}\le \news{\bm{0}}{\samplesize{1},0}+\news{\bm{0}}{0,\samplesize{2}}\le  2\max\{ \news{\bm{0}}{\samplesize{1},0},\news{\bm{0}}{0,\samplesize{2}}\}
    \end{align*}
    We can lower bound the left hand side by 
    \begin{align*}
        \max\{ \news{\bm{0}}{\samplesize{1},0},\news{\bm{0}}{0,\samplesize{2}}\}&\ge \max\{ \conc{1}\samplesize{1}^{\rate{}}, \conc{2}\samplesize{2}^{\rate{}}\}\ge \min\{\conc{1},\conc{2}\}\max\{\samplesize{1},\samplesize{2}\}^\rate{}\\
        &\ge 2^{-\rate{}}\min\{\conc{1},\conc{2}\} (\samplesize{1}+\samplesize{2})^\rate{}
    \end{align*}
    And the right hand sided can be upper bounded in a similar manner
    \begin{align*}
        2\max\{ \news{\bm{0}}{\samplesize{1},0},\news{\bm{0}}{0,\samplesize{2}}\}&\le 2\max\{\conc{1},\conc{2}\}\max\{\samplesize{1},\samplesize{2}\}^\rate{} \le 2\max\{\conc{1},\conc{2}\}(\samplesize{1}+\samplesize{2})^\rate{}
    \end{align*}

    Thus in this case we have $\news{\bm{0}}{\samplesize{1},\samplesize{2}}\sim C'(\samplesize{1}+\samplesize{2})^{\rate{}}$




\end{proof}

\begin{figure}
    \centering
    \includegraphics[width = 0.6\textwidth]{Figs/powerlaw_simu_.3_.6_.5.png}
    \caption{Simulated sampling curve with $\mass = 10, \rate{1}=0.3, \rate{2}=0.6, \conc{1}=\conc{2}=1, \corr{i}=\corr{2}=0.5$ in the projection scheme, i.e. sampling population 1 or population 2 only. The mean growth curves (shown in lines) were calculated using 100 independent realizations and a single realization is shown as dots. The bound for population 2 is 0.3 and 0.6 and the predicted power law rate for population 1 is 0.3. We fit the line using the last 1/3 of the mean growth curve. The fitted powerlaw align well with our theoretical prediction.}
\end{figure}


==> tex/power_law_main-old.tex <==
% !TEX root = ../double_trouble_main.tex

We next show that, for fixed hyperparameters, our model exhibits desirable power-law growth in the number of variants as a function of the number of samples. Recall that similar power-law behavior is widespread in natural systems. For instance, scientists have observed that the number of prognostic genes increases as a power of the number of sampled individuals \citep{li2023effect}. Outside of genetics, the number of observed species increases as a power of time or area of observation \citep{arrhenius1921species, connor1979statistics}; for a short period after first introduction into a country, the number of COVID-19 cases increases as a power of time \citep{manchein2020strong}; the number of homicide cases increases as a power of population size \citep{gomez2012statistics}. \citet{Broderick2012} refers to this type of power law as Type I, and the one-population 3BP is known to exhibit it \citep{teh2009indian,Broderick2012}.

In the two-population case, there are multiple different ways to grow the sample size -- depending on how one balances samples from the two populations. In what follows, we focus on two sampling schemes. In what we call the \emph{projection scheme}, we sample from exactly one of the two populations. In the \emph{proportional scheme}, we collect samples from the two populations according to some fixed proportion; in particular, for some constant $\propt > 0$, $N_1 =  \lceil\rho N_2\lceil$.

First, we demonstrate power-law growth, and bounds on power-law growth, for the projection scheme. In what follows, we will present symmetric results for each population, so we will find it useful to introduce the notation $\notpopidx$ for the other population besides $\popidx$; that is, when $\popidx = 1$, we have $\notpopidx = 2$ and vice versa. We use $\zerovec$ to represent a vector of zeros. In the next results, we write $a_\samplesizenosubscript \sim b_\samplesizenosubscript$ to indicate $\lim_{\samplesizenosubscript\to\infty} a_\samplesizenosubscript/b_\samplesizenosubscript=1$.
%%%
\begin{myProposition}[Power-law bounds under the projection sampling scheme] 
\label{prop:power_law_proj}
	\textcolor{orange}{
	Take a two-population model (\cref{eq:generative_model}) with our proposed PPP rate measure (\cref{eq:proposed_prior}) and hyperparameters
	$\mass, \conc{1}, \conc{2}, \corr{1}, \corr{2}>0$ and $\rate{1}, \rate{2} \in (0,1)$.
	Define $\rate{\popidx}'=\max\{\rate{\notpopidx}, \rate{\popidx}-\corr{\notpopidx}(\rate{\popidx}/\rate{\notpopidx}-1)\}$.
	Then there exist constants $C_1, C_2, C'_1, C'_2, \samplesize{1,0}, \samplesize{2,0}$ depending only on $\rate{1},\rate{2}$ such that, when $\rate{\popidx} \le \rate{\notpopidx}$, we have the following relationships.
	%
	\begin{equation} 
		 \label{eq:power-law_projection}
		\textrm{Fix } \samplesize{\notpopidx} = 0. \textrm{ Then }
		\news{\zerovec}{\vecsamplesize}
			\sim C_\popidx \samplesize{\popidx}^{\rate{\popidx}} \textrm{ a.s.\ as } \samplesize{\popidx} \rightarrow \infty.
	\end{equation}
	%
	And for any $\samplesize{\notpopidx} > \samplesize{\notpopidx,0}$,
	%
	\begin{equation}
		\label{eq:projection_bounds}
		\textrm{Fix } \samplesize{\popidx} = 0. \textrm{ Then }
		C'_{\notpopidx} \samplesize{\notpopidx}^{\rate{\notpopidx}'}
			\le \news{\zerovec}{\vecsamplesize}
			\le C_{\notpopidx} \samplesize{\notpopidx}^{\rate{\notpopidx}} \quad \text{a.s.}
	\end{equation}
	%
	}
\end{myProposition}

See \cref{sec:projection_scheme_proof} for the proof. 
Note that, due to the maximum in its definition, we expect $\rate{\popidx}'$ to always be lower bounded by $\rate{\notpopidx}$ and hence
strictly positive. So our bounds in \cref{eq:projection_bounds} are non-trivial.

\textcolor{orange}{
We see that we can prove that the population with the lower rate parameter 
exhibits Type I power law behavior where the power is exactly the rate parameter in that population. This behavior is reminiscent
of the one-population 3BP case, where the number of variants grows as a power of the number of samples, and the power 
is exactly the one-population rate parameter \citep{Broderick2012}. \textcolor{red}{TB: should we also cite teh and gorur for that last bit?}
Notably, despite the asymmetry of our PPP rate measure in \cref{eq:proposed_prior}, we do obtain symmetric roles for the rate
parameters across the two populations here; this symmetry inspires our use of the name \emph{rate parameter} in analogy
to the one-population case.
}

\textcolor{orange}{
For the population with the higher rate parameter, we are able to provide only a set of bounds on growth rather than the sort of 
exact asymptotic behavior we see in the one-population case or the case of the lower rate hyperparameter.
When the correlation parameters are sufficiently small, $\rate{\notpopidx}'$ will be nearly equal to $\rate{\notpopidx}$ and 
the power of $\samplesize{\notpopidx}$ on both sides of \cref{eq:projection_bounds} will nearly match. Conversely if the
correlation parameters are sufficiently large, the power in the lower bound of \cref{eq:projection_bounds} will be $\rate{\popidx}$.
}

\textcolor{orange}{
Our empirics in \cref{fig:power-law}
corroborate our theory and suggest we may not be able to replace \cref{eq:projection_bounds}
with the analogue of \cref{eq:power-law_projection}. In our experiment, population 1 has the lower rate parameter. 
We grow a single population at a time and set the number of samples in the other population to 0.
As expected, the number of variants in population 1 seems to be growing at a rate increasingly close to $\rate{1}=0.3$
as the number of samples grows.
Although our theory holds for any single realization (points in \cref{fig:power-law}), we also take a mean across 
100 independent realizations to smooth out noise (solid curves in \cref{fig:power-law}).
We regress the final third of the mean points in the log-log plot for population 1 to estimate the power at 0.34.
While our theory does not imply population 2 must follow a power law, we find empirically that it does seem
to exhibit a power law much like population 1. We empirically estimate the power as for population 1 and find 0.49.
Our theory eventually bounds the number of variants in population 2
by $C'_2 \samplesize{2}^{0.5}$ below and $C_2 \samplesize{2}^{0.6}$ above, for some $C'_2$ and $C_2$. 
Our empirical power value of 0.49 seems consistent with treating 0.5 and 0.6 as upper and lower bounds on power-law
behavior respectively when we consider the noise in this finite realization; cf.\ our results for population 1.
It seems less likely, though, that we can expect the population 2 power to exactly match the population 2 rate parameter since
0.49 is somewhat far from the upper bound rate of 0.6.
We conjecture that one may be able to show that the population with higher rate parameter does generally exhibit a Type I power 
law in the projection scheme, but the power need not exactly match the corresponding rate parameter.
}


\begin{figure}[htp] \label{fig:power-law}
    \centering
    \includegraphics[width = 0.6\textwidth]{Figs/powerlaw_simu_.3_.6_.1.png}
    \caption{Simulated sampling curve with $\mass = 10, \rate{1}=0.3, \rate{2}=0.6, \conc{1}=\conc{2}=1, \corr{1}=\corr{2}=0.1$ in the projection scheme, i.e., sampling population 1 or population 2 only. The mean growth curves were calculated by taking average of 100 independent realizations at each sample size. The line is by connecting all points of the average growth. A single realization is shown as dots. The theoretical lower and upper bound growth rate for population 2 is 0.5 and 0.6, respectively while the theoretical power law rate for population 1 is 0.3. We use the last 1/3 of the mean growth curve to fit the power law growth rate. The mean growth curve appear linear in log-log scale while the fitted power law rate for population 2 is 0.49 and population 1 is 0.34. }%\footnote{LM:I like the idea of having a figure to show the quality of the bound - I wonder whether we should have it here or later in the text though (e.g., within the synthetic experiments?) I also think we should describe it in more depth - what is the simulation? how many samples? how many times did we draw from the model for a single configuration of the hyperparameters? \yunyi{Aha good catch, the details are in the appendix but we can get it eariler}}
\end{figure}

We highlight the special case of equal rate hyperparameters in the following corollary. In this case, we can give the exact asymptotic behavior in the projection scheme
as either population grows.

\begin{myCorollary}
    \label{coro:power-law-rate-align}
    Take the same assumptions as \cref{prop:power_law_proj}. Further take $\rate{1}=\rate{2}=\rate{}$. For either $\popidx$, fix $\samplesize{\notpopidx} = 0$. Then
    	$\news{\zerovec}{\vecsamplesize} \sim C_\popidx \samplesize{\popidx}^{\rate{}} \text{ a.s.}$ as $\samplesize{\popidx} \to \infty$. 
\end{myCorollary}
\begin{proof}
   The result follows from \cref{eq:power-law_projection}. We observe that \cref{eq:projection_bounds} simultaneously applies -- with the roles of $\popidx$ and $\notpopidx$ switched -- and offers no contradiction.
\end{proof}

 
One way the proportional scheme arise is when one samples two populations at random then asymptotically both $N_1,N_2\to\infty$ while the ratio between two sample sizes approach the a fixed constant depends on proportion of population 1 and 2 in the total population. When the population labels are not observed but exist, the sample can be a random sample thus asymptotically follow a proportional design and we expect our model to show some power law behavior between total number of variants seen and total number of samples taken in such case. \Cref{coro:proportional} establishes that in proportional sampling scheme, the total number of variants seen as a function of total number of samples $N_1+N_2$ can be lower and upper bounded by power law growth. %\Cref{coro:rate_align} showed that when the two rate parameters are the same, instead of having power law lower and upper bounds, we have power law growth for both populations.  

\begin{myCorollary}[Powerlaw bounds proportional scheme] 
    \label{coro:proportional}
    For the proposed model~\Cref{eq:generative_model} %\footnote{LM: I think again having an equation with the exact model we are referring to would be helpful; this is kind of informal (especially within a ``theorem'' environment imo) /\yunyi{I hear that}} 
with $\rate{1},\rate{2}\in(0,1)$, for some constant $C_3,C_4$ not depending on $\samplesize{1}, \samplesize{2}$ (where $\samplesize{2}=\propt\samplesize{1}$), we have when $\rate{1}\le \rate{2}$ and $\rate{2}-\corr{1}(\rate{2}/\rate{1}-1)\in (0,1)$, as $\samplesize{1}, \samplesize{2}\to\infty$
    \begin{align*}
        C_3(\samplesize{1}+\samplesize{2})^{\max\{\rate{1},\rate{2}-\corr{1}(\rate{2}/\rate{1}-1)\}}&\le \news{\bm{0}}{\samplesize{1},\propt\samplesize{1}}\le C_4(\samplesize{1}+\samplesize{2})^{\max\{\rate{1},\rate{2}\}} \text{    a.s.}
    \end{align*}
    where $C_3\ge \frac{\min\{C_1,C_2\propt^{\rate{2}}\}}{(1+\propt)^{\max\{\rate{1},\rate{2}-\corr{1}(\rate{2}/\rate{1}-1)\}}}$ and $C_4\le 2\max\{C_1,C_2\propt^{\rate{2}}\}(1+\propt)^{-\max\{\rate{1},\rate{2}\}}$ and $C_1$, $C_2$ are the constants in~\eqref{eq:power-law-pop1} and~\eqref{eq:power-law-pop2} respectively.
\end{myCorollary}
The proof is given in~\Cref{sec:proportion_scheme_proof}. The idea is to use the fact in a sample with both populations, the number of variants seen is lower bounded by the number of variants seen in either population and upper bounded by sum of the variants seen in both populations (i.e. the double counted number), then apply power-law bounds in~\Cref{prop:power_law_proj}.

\begin{myCorollary}[Power-law when rate align]
    \label{coro:rate_align}
    For the proposed model with $\rate{1}=\rate{2}=\rate{}\in(0,1)$, for some constant $C'$ does not depends on $\samplesize{1},\samplesize{2}$, we have as $\samplesize{1}, \samplesize{2}\to\infty$
    \begin{align*}
        \news{\bm{0}}{\samplesize{1},\samplesize{2}}\sim C'(\samplesize{1}+\samplesize{2})^\rate{}\text{    a.s.}
    \end{align*} 
    where $C'\ge 2^{-\rate{}}\min\{C_1,C_2\}$  and $C'\le 2\max\{C_1,C_2\}$ with $C_1$, $C_2$ being the constants in~\eqref{eq:power-law-pop1} and~\eqref{eq:power-law-pop2} respectively.
\end{myCorollary}

The proof is essentially apply power law rate in \Cref{coro:power-law-rate-align} and was given in~\Cref{sec:two_rate_the_same}. 
%\footnote{LM: I generally like avoiding extra notation, but it seems like the expression $\rate{2}-\corr{1}(\rate{2}/\rate{1}-1)$ (and its symmetric counterpart where the roles of pop 1 and 2 are inverted) comes up often. maybe worth considering introducting a new parameter $\rho_{1,2}$ or something? Also worth discussing why this comes up and what it represents somewhere? \yunyi{Really good catch on what it represents, I kind of understand it as some kind of balance between power-law and correlation between two populations let me mark it as a big TODO.}}

%\begin{myRemark}
%    The proportional scheme arguably being the most common scheme when population labels are not observed. Our result suggest in this case our prior model will still have power-law bounds and the rate depends on the fastest population. Actually, the two corollaries only relies on the results proposition~\ref{prop:power_law_proj} and could be used in other models. \footnote{LM: what are we trying to convey via this remark?}
%\end{myRemark}



==> tex/spp_sampling_2d.tex <==
As a preparation of checking the behavior of our prior, we need to extend theory developed in \citet{Broderick2012} and \citet{Gnedin2007} to multiple dimensions. That is, suppose we sample species from two or more populations that are different but share the same species pool thus species labels are shared and matched. The rate for species $i$ will then be a vector $\bm{p}_i=(p_1,\dots, p_J)$ for $J$ populations where $J<\infty$ is fixed (which can be extended). A box and ball analogy is there are infinite amount of boxes and we have colored balls to put in, with different probabilities. 

We first introduce some notations. We define $K_{N}$ for $N=(N_1,\dots,N_J)$ being the number of features in a sample of size $(N_1,\dots,N_J)$, and $K_{N,r}$ the number of features repeated $r=(r_1,\dots,r_J)$ times in a sample of $N=(N_1,\dots, N_J)$ follow \citet{Gnedin2007, Broderick2012}, we work with the expectations. Define
\begin{equation}
    \label{eq:number_of_feature}
    \Phi_N:=\E K_N \text{  and  } \Phi_{N,r}:=\E K_{N,r} \text{  }(\sum_j r_j>0)  
\end{equation}

Analyses are similar for multiple population extension of 1) \citet{Broderick2012} where $X_{i,j,n_j}\sim \text{Binomial}(p_{i,j})$ for $j=1,\dots,J$ where we have a CRM prior on $\bp_{i}$'s and $\nu(\bp)$ is a Poisson rate measure, and 2)\citet{Gnedin2007} where we have $X_{j,n_j}\sim\text{Multinomial}(p_{1,j},\dots)$ and $\nu(\bp)=\sum_i \delta_{\bp_i}$. We can interpret both be a L\'evy measure. Since $N$ is a vector, there are many way to send $N\to\infty$, we will mainly work with sequence of sample size $N_\ell$ such that $N_{j,\ell}\le N_{j,\ell+1}$ for all $j=1,\dots,J$ and $\ell \ge 1$. 

\subsection{Poissonization}

We follow the principle discussed in \citet{Gnedin2007}, that is, we consider a \textit{Poissonized} version of the sampling process by defining independent Poisson process with rate $p_{i,j}$'s (the rate of population $j$ of atom $i$). 

we define $K(t)$ and $K_{r}(t)$'s by constructing Poisson process on the positive line, one for each feature. Then $K(t)$ will be number of such process $K_r(t)$ will be the number of Poisson process with $r$ points. Take $\bp_i$'s to be a enumeration of the (vector-valued) atom weight, we assume they are a random weight coming from some Poisson process with rate measure $\nu(d\bp)$ that satisfy the finite expectation requirement. We only assume they are strictly positive and each coordinates sum to finite $\sum_i  p_{i,j}<\infty$ for all $j$ (and $\sum_i  p_{i,j}=1$ for the DP case). 

We take $\Pi_{i,j}$ to be a standard Poisson with rate $p_{i,j}$ $\Pi=\bigcup_{i,j} \Pi_{i,j}$ is itself a Poisson process. We can define:
\begin{align*}
    K(t):=\sum_i I\left\{  \sum_{j=1}^J \vert\Pi_{i,j}\cap [0,t_j]\vert>0\right\}
\end{align*}
and
\begin{align*}
    K_r(t):=\sum_i \prod_{j=1}^J I\left\{  \vert\Pi_{i,j}\cap [0,t_j]\vert=r_j\right\}
\end{align*}

Since $\bp$ are random, the Poissonized version allowed us to write
\begin{align*}
    \Phi(t)=\E K(t)=\E\left[\E\left[K(t)\vert \bp\right]\right]=\E\left[\E\left[\sum_i I\left\{  \sum_{j=1}^J \vert\Pi_{i,j}\cap [0,t_j]\vert>0\right\}\vert \bp\right]\right]
\end{align*}
Condition on $\bp$ the two Poisson processes are independent, thus we can have
\begin{align*}
    \Phi(t)=\E\left[\sum_i\left(1-e^{-\sum_{j=1}^J p_{i,j}t_j}\right)\right] 
\end{align*}
Similarly, 
\begin{align*}
    \Phi_r(t)=\E\left[\prod_{j=1}^J \frac{(t_jp_{i,j})^{r_j}}{r_j!}e^{-t_jp_{i,j}}\right]
\end{align*}

Apply Campbell's Theorem, we have
\begin{align}
    \Phi(t)&=\E\left[\sum_i\left(1-e^{-\sum_{j=1}^J p_{i,j}t_j}\right)\right] =\int_{[0,1]^J}\left(1-e^{-\sum_{j=1}^Mp_{j}t_j}\right)\nu(d\bp)\label{eq:poised_feature}\\
    \Phi_N&=\E\left[\sum_i\left(1-\prod_{j=1}^J(1-p_{i,j})^{N_j}\right)\right]=\int_{[0,1]^J}\left(1-\prod_{j=1}^J(1-p_{j})^{N_j}\right)\nu(d\bp) \label{eq:expect_total_feature}\\
    \Phi_r(t)&=\E\left[\sum_i\prod_{j=1}^J \frac{(t_jp_{i,j})^{r_j}}{r_j!}e^{-t_jp_{i,j}}\right]=\int_{[0,1]^J}\prod_{j=1}^J \frac{(t_jp_{j})^{r_j}}{r_j!}e^{-t_jp_{j}}\nu(d\bp)\label{eq:poised_rton}\\
    \begin{split}
        \Phi_{N,r}&=\left[\prod_{j=1}^J\binom{N_j}{r_j}\right]\E\left[\sum_i\prod_{j=1}^J p_{i,j}^{r_j}(1-p_{i,j})^{N_j-r_j}\right]\\
    &=\left[\prod_{j=1}^J\binom{N_j}{r_j}\right]\int_{[0,1]^J}\prod_{j=1}^J p_{j}^{r_j}(1-p_{j})^{N_j-r_j}\nu(d\bp)
    \label{eq:expect_rton}
    \end{split}
\end{align}

These are multiple population extensions of Equations (9)-(12) of \citet{Gnedin2007}. The summability assumption $\sum_i p_{i,j}<\infty$ (resp. $sum_i p_{i,j}=1$) will translate to $\int_{[0,1]^J} p_j \nu(d\bp)<\infty$ (resp. $\int_{[0,1]^J} p_j \nu(d\bp)=1$). Recall we also have $\int_{[0,1]^J} \nu(d\bp)=\infty$. 

\subsection{Estimation of moments}

\begin{myProposition}[Sublinear diverging]
    we have $\Phi(t)\to\infty$ and $\Phi_N\to\infty$ a.s. with $\max_j N_j\to\infty$. But $\Phi_N\ll \max_j N_j$ and $\Phi(t)\ll \max_jt_j$. 
\end{myProposition}
\begin{proof}
    First part is by Monotone convergence on Equations~\eqref{eq:poised_feature} and~\eqref{eq:expect_total_feature} (recall we only allow $N_j$'s (resp. $t_j$'s) to increase).

    We consider the first $I$ species already seen, the mean number of species to be discovered is at most
    \begin{align*}
        \Phi_N<I+\sum_{j=1}^J N_j \sum_{i> I} p_{i,j} \le I+\left(\max_{j} N_j\right)\left(\sum_{j=1}^J\sum_{i> I} p_{i,j}\right)
    \end{align*}
    By the assumption $\sum_i p_{i,j}<\infty$ and take $I$ arbitrarily large. Apply the same argument to $\Phi(t)$ we have
    \begin{align*}
        \limsup \frac{\Phi_N}{\max_j N_j}=\limsup \frac{\Phi(t)}{\max_j t_j}=0
    \end{align*}
\end{proof}

We proceed estimating errors by Poissonization. 

\begin{myLemma}[Poissonization error]
    For the Poissonized estimation We have
    \label{lemma:poissonization}
    \begin{align}
        \vert \Phi(N)-\Phi_N \vert &< 2\frac{\Phi(N)}{\max_j N_j}\to 0 \text{  as  } \max_j\{N_j\}\to\infty\\
        \vert \Phi_r(N)-\Phi_{N, r} \vert &< 2c\frac{\Phi(N)}{\max_j N_j}\to 0 \text{  as  } \min_{j:N_j>0}\{N_j\}\to\infty
    \end{align}
\end{myLemma}
\begin{proof}
    We use the elementary inequality $0\le e^{-Np}-(1-p)^N\le N p^2 e^{-Np}$ for $p\in(0,1)$, we have for any $j$
    \begin{align*}
        0\le e^{-\sum_j p_jN_j}-\prod_j (1-p_j)^{N_j}\le e^{p_jN_j}-(1-p_j)^{N_j}\le N_j p_j^2 e^{-Np_j}
    \end{align*}
    Thus we take $j$ to be the one that $N_j$ is the maximum, 
    \begin{align*}
        \vert \Phi(N)-\Phi_N \vert &= \int_{[0,1]^J} \left(e^{-\sum_j p_jN_j}-\prod_j (1-p_j)^{N_j}\right)\nu(d\bp)\\
        &\le N_j \int_{[0,1]^J} p_j^2 e^{-N_jp_j} \nu(d\bp)=\frac{2}{N_j}\Phi_{2e_j}(N_j)\\
        &\le \frac{2}{\max_j N_j}\Phi(N)\to 0\\
    \end{align*}
    In which we denote $2e_j$ as the vector that only $j$th entry is 2 and 0 otherwise, then the second equal is because Equation~\eqref{eq:expect_rton}, the last line is because of our choice of $j$. 
    
    For the second estimation we first observe that for $j$'s that $N_j=0$ it will not contribute to the estimation so we focus on the $j$'s such that $N_j>0$. The same calculation carry through when $\binom{N_j}{r_j}$ approximates $\frac{N_j^{r_j}}{r_j!}$, this will happen when $N_j\to\infty$, thus we require $\min_{j:N_j>0} N_j\to\infty$ in the second line. 
\end{proof}

\subsection{Law of large numbers}

We would like that with $N\to\infty$ in some way we have some LLN type of results as in \citet{Broderick2012}'s proposition 6.4 (for beta processes) and \citet{Gnedin2007}'s proposition 2 (for Dirichlet processes) showing $K_N$ close to $\Phi_N$. We rely on Borel-Cantelli lemma.

\begin{myLemma}[Large deviation bound and Law of Large Numbers]
    \label{lemma:LLN}
Suppose $\exp(-\epsilon'\Phi_{N_\ell})$ is summable for any $\epsilon'>0$ for an increasing sequence of sample size vector $\{N_\ell\}_{\ell=1}^\infty$ such that $N_{j,\ell}\le N_{j,\ell+1}$ for all $j,\ell$ (i.e. we always take more samples), we have $K_{N_\ell}\to \Phi_{N_\ell}$ a.s. as $\ell\to\infty$. Further, if $\exp(-\epsilon'\Phi_{N_\ell,s})$ is sumable for some given fixed integer vector $s\in \mathbb{N}_+^M$, $\sum_{\{r:r_j\ge s_j\}}K_{N_{\ell},r}\to \sum_{\{r:r_j\ge s_j\}}\Phi_{N_{\ell},r}$ a.s..
\end{myLemma}
\begin{proof}
    Follow the same argument as in \citet{Broderick2012} and \citet{Gnedin2007}. We apply \citet[pp.911, Theorem 4]{Freedman1973}, for any given $\epsilon>0$, we have some $\epsilon'$ depends only on $\epsilon$ and some constant $c$  such that
    \begin{align*}
        P\left(\lvert\frac{K_{N_\ell}}{\Phi_{N_\ell}}-1\lvert\ge \epsilon\right)<ce^{-\epsilon'\Phi_{N_\ell}}
    \end{align*}
    By assumption we have
    \begin{align*}
        \sum_{\ell\to\infty} P\left(\lvert\frac{K_{N_\ell}}{\Phi_{N_\ell}}-1\lvert\ge \epsilon\right)<\infty
    \end{align*}
    By Borel-Cantelli we have $K_{N_\ell}/\Phi_{N_{\ell}}\to 1$ a.s.. The second follow the same result observing $\sum_{\{r:r_j\ge s_j\}} K_{N_{\ell},r}$ is monotone. 
\end{proof}

\begin{myRemark}
    The above result is on $N_\ell$, but when we would like to understand the tail behavior we will actually work on the Poissonized version and make use of the result in Lemma \ref{lemma:poissonization}. 
\end{myRemark}

\subsection{Tail behaviors}
With Lemma~\ref{lemma:poissonization} and~\ref{lemma:LLN} in hand, we can focus our investigation of the tail behavior on $\Phi(t)$ and $\Phi_r(t)$. We will need some extended notion of tail behavior in \citet{Broderick2012} and \citet{Gnedin2007}. However in $\R_+^J$ there are multiple sets can be view as ``tail'' while Lemma~\ref{lemma:poissonization} provide some insight on which set we have good estimate.

We will consider two different tails for different requirement in Lemma~\ref{lemma:poissonization}. The first case we refer here after as \textit{maximum} tail is $\Tcal_{\max}(x)=\R_+^J\setminus[0,x]^J $ with $x\to\infty$ where we must have $\max_j N_j\to\infty$ if $N\in \Tcal_{\max}(x)$ as $x\to\infty$ and the second we refer as \textit{minimum} tail $\Tcal_{\min}(x)=[x,\infty)^J$ where we have $\min_j N_j\to\infty$ if $N\in \Tcal_{\min}(x)$ and $x\to\infty$ (see Fig.\ref{fig:tail} for an illustration in $\R_+^2$). 
\begin{figure}[htp]
    \centering
\begin{tikzpicture}
    \filldraw[black!30, thick] (0,0) rectangle (3,3);
    \draw[black, thick] (0,0) rectangle (3,3);
    \filldraw[white, thick] (0.05,0.05) rectangle (2,2);
    \draw[black, thick] (4,0) rectangle (7,3);
    \filldraw[black!30, thick] (6,2) rectangle (7,3);
\end{tikzpicture}
\caption{Illustration of two tails in $\R^2_+$. Shad area represent the tail area. Left: the maximum tail, Right: the minimum tail. }
\label{fig:tail}
\end{figure}

Recall $\nu$ is a measure, we denote
\begin{align}
    \nu_{\min}(x)&=\nu(\Tcal_{\min}(x))\\
    \nu_{\max}(x)&=\nu(\Tcal_{\max}(x))
\end{align}


